Representation Learning for Frequent Subgraph Mining

Identifying frequent subgraphs, also called network motifs, is crucial in analyzing and predicting properties of real-world networks. However, finding large commonly-occurring motifs remains a challenging problem not only due to its NP-hard subroutine of subgraph counting, but also the exponential growth of the number of possible subgraphs patterns. Here we present Subgraph Pattern Miner (SPMiner), a novel neural approach for approximately finding frequent subgraphs in a large target graph. SPMiner combines graph neural networks, order embedding space, and an efficient search strategy to identify network subgraph patterns that appear most frequently in the target graph. SPMiner first decomposes the target graph into many overlapping subgraphs and then encodes each subgraph into an order embedding space. SPMiner then uses a monotonic walk in the order embedding space to identify frequent motifs. Compared to existing approaches and possible neural alternatives, SPMiner is more accurate, faster, and more scalable. For 5- and 6-node motifs, we show that SPMiner can almost perfectly identify the most frequent motifs while being 100x faster than exact enumeration methods. In addition, SPMiner can also reliably identify frequent 10-node motifs, which is well beyond the size limit of exact enumeration approaches. And last, we show that SPMiner can find large up to 20 node motifs with 10-100x higher frequency than those found by current approximate methods.

==> ack.tex <==
\section{Acknowledgement}
We gratefully acknowledge the support of
DARPA under Nos. FA865018C7880 (ASED), N660011924033 (MCS);
ARO under Nos. W911NF-16-1-0342 (MURI), W911NF-16-1-0171 (DURIP);
NSF under Nos. OAC-1835598 (CINES), OAC-1934578 (HDR), CCF-1918940 (Expeditions), IIS-2030477 (RAPID);
Stanford Data Science Initiative, 
Wu Tsai Neurosciences Institute,
Chan Zuckerberg Biohub,
Amazon, Boeing, Chase, Docomo, Hitachi, Huawei, JD.com, NVIDIA, Dell. 
J. L. is a Chan Zuckerberg Biohub investigator.



==> content/borader_impact.tex <==
\newpage
\section{Broader Impact}
Network motif analysis is widely applied in diverse domains from biology and chemistry to the social sciences~\cite{agrawal2018large,cereto2015molecular,leskovec2010signed}, for both exploratory data analysis and predictive modeling. Our research could be used to identify frequent motifs to facilitate scientific research in characterizing the important substructures in a graph dataset. As a frequent motif mining method, \name\ can help to partially automate the scientific process of understanding a new dataset by identifying promising graph structures for further analysis. Traditional methods for this problem have shown success in identifying important chemical and social substructures~\cite{ketkar2005subdue}; \name\ has the potential to do the same for larger motifs than previously possible, which could facilitate new scientific discoveries.

However, frequent motif mining methods have their caveats. Their rigorous objective function, while enabling objective interpretation of model outputs, does not necessarily translate to identifying motifs with high scientific importance. Broadly, automated motif mining methods carry the risk of automation bias, or undue trust in model predictions. If such methods are implemented in general data analysis systems without proper explanation, they risk being used by those who do may too optimistically interpret the method's output, leading to incorrect scientific results. As a neural system, \name\ carries the additional risks of decreased interpretability and systematic bias in model predictions.

Despite these caveats, neural motif mining methods have the potential to greatly assist human scientific discovery. To mitigate associated risks, we encourage research to understand how users interact with motif mining and other data exploration tools. Can such tools accelerate exploration of scientific hypotheses without increasing automation bias?

%GNNs (and hence GNNExplainer) could be applied to a wide range of applications, including computer vision, natural language processing, recommender systems, traffic prediction, generative models and many more (Zhou et al 2019, Wu et al 2019). Our research could be used to provide explanations for GNNs in these applications, improving understanding of individual decisions, as well as the underlying models.
%While there will be important impacts resulting from the use of GNNs in general, here we focus on the impact of using our tool to provide explanations for such systems. There are many benefits to using such a tool, such as increasing the transparency in decision-critical applications. This can help mitigate fairness, privacy and safety risks — see the introduction of the paper for more details. The potential risks of increasing explainability have typically received less attention. These include: (i) the risk of automation bias, i.e. an undue trust in models (see e.g. PAI 2019), (ii) if the use of explanations means systems may now be used by those with lower levels of domain or ML expertise, this could increase the risk of the model or its outputs being used incorrectly, (iii) if explanations are only used during the development phase, and the model is retrained over time, changing its behaviour, this could again lead to a false sense of security.
%We see opportunities for research applying GNNExplainer to beneficial purposes, such as investigating whether GNNExplainer could improve algorithmic fairness. To mitigate the risks associated with using generated explanations, we encourage research to understand the impacts of using GNNExplainer in particular real-world scenarios. In these scenarios, do users understand the explanations given, and act accordingly, not falling prey to automation bias? Does use of the system improve or diminish domain expertise over time?

==> macros.tex <==
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{url}
\usepackage{verbatim} % allows multiline comments
\usepackage{graphicx}
% \usepackage{caption} 
\usepackage{multirow}
\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{xspace}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{times}
\usepackage{xr}
\usepackage{bbm}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{hyperref}       % hyperlinks
\usepackage{multicol}
\usepackage{tabularx}
\usepackage{perpage} %the perpage package
\MakePerPage{footnote} %the perpage package command
\usepackage{wrapfig}

\newcommand{\andrew}[1]{{{\textcolor{teal}{[Andrew: #1]}}}}
\newcommand{\rex}[1]{{{\textcolor{magenta}{[Rex: #1]}}}}
\newcommand{\jure}[1]{{{\textcolor{red}{[Jure: #1]}}}}


\newcommand{\xhdr}[1]{{\noindent\bfseries #1}.}
\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\CITE}{{\textcolor{red}{[CITE]}}}

\newcommand{\nedge}{k}
\newcommand{\mb}{\mathbf}
% \newcommand{\mc}{\mathcal}
\newcommand{\cut}[1]{}
%\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}
\newcommand{\casc}{{\mathbf{t}}}
\newcommand{\alphs}{{\mathbf{A}}}
\newcommand{\xsketch}{\noindent {\it Proof Sketch.}}
\newcommand{\netinf}{{\textsc{Net\-Inf}}\xspace}
\newcommand{\multitree}{{\textsc{Multi\-Tree}}\xspace}
\newcommand{\netrate}{{\textsc{Net\-Rate}}\xspace}
\newcommand{\connie}{{\textsc{Co\-nNIe}}\xspace}
\newcommand{\maxinf}{{\textsc{Max\-Inf}}\xspace}
\newcommand{\expo}{{\textsc{Exp}}\xspace}
\newcommand{\pow}{{\textsc{Pow}}\xspace}
\newcommand{\ray}{{\textsc{Ray}}\xspace}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}

\newcommand{\name}{BiDyN\xspace}

